A convex relaxation to compute the nearest structured rank deficient matrix

Given an affine space of matrices $\mathcal{L}$ and a matrix $\Theta\in \mathcal{L}$, consider the problem of computing the closest rank deficient matrix to $\Theta$ on $\mathcal{L}$ with respect to the Frobenius norm. This is a nonconvex problem with several applications in control theory, computer algebra, and computer vision. We introduce a novel semidefinite programming (SDP) relaxation, and prove that it always gives the global minimizer of the nonconvex problem in the low noise regime, i.e., when $\Theta$ is close to be rank deficient. Our SDP is the first convex relaxation for this problem with provable guarantees. We evaluate the performance of our SDP relaxation in examples from system identification, approximate GCD, triangulation, and camera resectioning. Our relaxation reliably obtains the global minimizer under non-adversarial noise, and its noise tolerance is significantly better than state of the art methods.

==> additionalproofs.tex <==
\section{Additional proofs}\label{s:additionalproofs}

\begin{lemma}\label{thm:idealsequal}
  $\mathcal{J}=\mathcal{J}'$, where
  $\mathcal{J}' := \langle p_i^T x,\; x^TE x - 1,\; x_{l_1}x_{l_2}-x_{l_3}x_{l_4} \rangle.$
\end{lemma}
\begin{proof}
  It is clear that $\mathcal{J}\subset \mathcal{J}'$.
  Let us prove now that $\mathcal{J}'\subset \mathcal{J}$.
  First notice that the rank one equations $x_{l_1}x_{l_2}-x_{l_3}x_{l_4}$ imply that
  $$x^T(p_ie_j^T)x \equiv_\mathcal{J} x^T\sym(p_ie_j^T)x\equiv_\mathcal{J} 0,$$
  and thus $(p_i^Tx)x_j \in \mathcal{J}$.
  Note that the entries of $x$ can be indexed by pairs $(j_1,j_2)$ with $0\leq j_1\leq n$, $1\leq j_2\leq k$.
  Observe that
  \begin{align*}
    p_i^T x \equiv_\mathcal{J} (p_i^Tx)(x^TEx) = \sum_{j_2} (p_i^Tx)x_{(0,j_2)}^2 \equiv_\mathcal{J} 0,
  \end{align*}
  and thus $p_i^T x \in \mathcal{J}$, as wanted.
\end{proof}

\begin{proof}[Proof of \Cref{thm:isomorphism}]
  Consider the map $\phi: \RR[x]/\mathcal{J}' \to \RR[v,z]/\langle{h}\rangle \to $ such that
  $f(x)\mapsto g(v,z):=f(\vone\otimes z)$.
  It is easy to see that $\phi$ is a well-defined homomorphism.
  Moreover, it is an isomorphism, whose inverse map is
  $g(v,z)\mapsto f(x):=g(\bar{v}(x),\bar{z}(x))$
  where
  $
    \bar{z}_{j}(x) := x_{(0,j)}$  and $ \bar{v}_i(x) := \sum_{j} x_{(i,j)}x_{(0,j)}.
  $
\end{proof}

\begin{proof}[Proof of \Cref{thm:quadraticforms}]
  Let $\RR[t]_d$ be the space of forms of degree~$d$ in $k$ variables.
  Observe that $\RR^k, \SS^k$ are in correspondence with $\RR[t]_1,\RR[t]_2$.
  The first item follows by noticing that if some linear forms $\{\ell_i(t)\}_i$ span $\RR[t]_1$ then $\{t_j \ell_i(t)\}_{ij}$ span $\RR[t]_2$.
  For the second item, it is clear that $\zeta\zeta^T \in L_2^\perp$, so it suffices to see that $\{\zeta\zeta^T\} \cup L_2 $ span $\SS^k$.
  This corresponds to the simple fact that if $\{\hat{\ell}\}\cup \{\ell_i(t)\}_i$ span $\RR[t]_1$ then $\{\hat{\ell}^2\}\cup \{t_j \ell_i(t)\}_{ij}$ span $\RR[t]_2$.
\end{proof}

